Sequence-Aware Recommender Systems

Recommender systems are one of the most successful applications of data mining and machine learning technology in practice. Academic research in the field is historically often based on the matrix completion problem formulation, where for each user-item-pair only one interaction (e.g., a rating) is considered. In many application domains, however, multiple user-item interactions of different types can be recorded over time. And, a number of recent works have shown that this information can be used to build richer individual user models and to discover additional behavioral patterns that can be leveraged in the recommendation process. In this work we review existing works that consider information from such sequentially-ordered user- item interaction logs in the recommendation process. Based on this review, we propose a categorization of the corresponding recommendation tasks and goals, summarize existing algorithmic solutions, discuss methodological approaches when benchmarking what we call sequence-aware recommender systems, and outline open challenges in the area.

==> domains.tex <==
\section{Application domains and datasets}
\label{sec:domains}
In this Section, we review the most important application domains of Sequential Recommendation. We then provide an overview on the publicly available datasets that can be used by researchers in this field. We believe this could be a useful resource for practitioners interested into specific application domains and for researchers who are looking for datasets for they experiments.

\subsection{Application domains}
In many domains the sequentiality of user interactions reveal very important characteristics of users' behavior that can be leveraged at recommendation time to help the user in fulfilling the desired goal. An overview of the application domains and of the most salient applications of sequential recommendation in each of them follows.
\begin{itemize}
\item \textit{E-commerce.} Sequential recommendation in e-commerce answers to questions like `what product(s) will the user buy next?' and `when the user will most like such product(s)?'. Sequential dependencies frequently show up between products bought by users. For example, a product and its replacement parts are usually bought in sequence, as well as a product and its accessories, as we have described in \autoref{sec:scenarios}. Additionally, the time interval between such subsequent interactions can be reliably extracted from users' historical data and used to make recommendations at the right time \citep{zhao12intervals,zhao14clusters}. Sequential purchase behaviors are relevant also for basket recommendation, whose goal is to recommend the set of few products the user will likely purchase next \citep{rendle10FPMC,wang15basket,yu16dynamic}. Finally, e-commerce platforms frequently deal with new and unregistered users. Providing effective recommendations to these users is crucially important to increase the chances of conversion, but it is definitely not a trivial task due to the lack of historical data. One valuable option is to use a session-based approach based on the sequential activity of the user in her current (and only) session \citep{hidasi16session,hidasi16feature}.
\item \textit{Web browsing.} Browsing within web pages is a strictly sequential process. SRSs can be employed to mine navigational patterns (\autoref{algo:fpm}) with the goal of (i) helping the user in her browsing by suggesting the following links or pages to open given her recent activity and (ii) pre-fetching web pages that will be likely opened next \citep{mobasher02sequential,nakagawa03impact,shani05mdp,yap12sequential,zhou04intelligent,zidmars01temporal}.
\item \textit{Query.} The goal of query suggestion is to find queries related with the previously issued ones \citep{baezayates04query}. Related queries can be successfully identified by extracting the intent of the user from the sequence of recent queries, for example, by using Markov models or Recurrent Neural Networks (\autoref{sec:sequence_learning}) \citep{he09query,sordoni15hierarchical}.
\item \textit{Locations.} Traveling is another strictly sequential process, since persons move from one place to another according their personal travel interests and goals. User movements are bounded by distance/time constraints (how long does it take to reach a specific place from the current position of the user?) and budget ones (how much does it cost to reach it?). For these reasons, models for sequential recommendation of locations jointly model the sequential relationship between locations sequential relationships between locations and the aforementioned constraints \citep{cheng13where,du16recurrent,feng15personalized,he16fusing,he16inferring,lian13checkin,lim15personalized,liu16next,liu16unified} Finally, location recommendation can be extended to actual tour recommendation, where a whole sequence of location is recommended according to the user's interests and constraints \citep{lim15personalized}.
\item \textit{Music.} In music listening transitions between songs are not as sharply defined as in many other domains. In fact, given the recent listening activity of the user, there are usually many equally good candidates to be played next that will equally please the user. However, transitions should obey to specific musicological constraints. These make certain transitions between pairs of songs more likely than others, and can be effectively modeled with Markov models (\autoref{sec:sequence_learning}) \citep{mcfee11nlp} and song embeddings (\autoref{sec:embeddings}) with \citep{vasile16meta} and without metadata \citep{chen12embedding,chen13multispace,wu13karaoke}. Listening tastes depend on many contextual factors -- such as -- mood that cannot be represented explicitly but instead must captured directly from the user's activity. Contextual music recommendation is therefore another interesting scenario of application of sequential recommendation \citep{hariri12context,hosseinzadeh15adapting,jannach15playlist,natarajan13app,turrin15large}. Finally, playlist recommendation is a natural sequence recommendation scenario. Almost every of the aforementioned techniques for next-song recommendation can be used to generate playlists. Playlist recommendation can be also presented as a constraint satisfaction problem, in which the list of songs that are recommended should satisfy a list of musicological and user defined constraints \citep{pauws06fast}.
\item \textit{Others.} Other domains in which sequential recommendation had beneficial impacts on the recommendation quality are \textit{news} and \textit{app} recommendation. News preferences are usually subject to trends, and visitors of online newspapers are often casual readers with a short browsing history. This is definitely a good application scenario for session-based recommendation based on sequence learning methods \citep{garcin13news}. App usage is another strongly contextual scenario that can severely benefit from the adoption of sequential recommendations to predict the apps that will most likely opened next for recommendation and prefetching applications \citep{baezayates15next}.
\end{itemize}

\subsection{Datasets}

\todo{Move this subsection to Evaluation section}

Many different publicly available datasets can be used for the goals of sequential recommendation. This is indeed a great advantage for researchers, who have many resources for testing their solutions and sharing their results with the community.  In principle, any dataset with a time-stamp attribute can be converted into sequential dataset. However, we must point out that not every dataset that complies with the previous property may be adequate for the purposes of sequential recommendations as we have described it throughout this survey. The reason is that some dataset -- such as the famous Netflix and Movielens datasets -- do not record actual user interactions, but instead they record the time at which the user provided her feedback, which might significantly differ from the time at which she actually interacted with an item. For example, users can rate a movie hours, or even days or weeks, after having watched it. While this is still a valuable source of information for time-aware recommender systems \citep{koren09cf}, whose goal is to model the long term dynamics in users' behavior, we believe this data is not adequate for the purposes of sequential recommendation, which focuses more on the immediate impacts of user interactions on her future behavior.

In \autoref{tab:datasets} we report the main characteristics of the publicly available datasets used by the papers analyzed in this survey. Please notice that this is not meant to be a comprehensive list of all the available datasets for sequential recommendation. Nevertheless, we believe it is still a valuable resource for researchers and practitioners interested in the field.

\begin{comment}
\begin{sidewaystable}
\caption{Publicly available datasets for sequential recommendation. An updated version of this table complete with URLs is available at this link [ TODO: ADD LINK].}
\label{tab:datasets}
\footnotesize
\begin{tabular}{P{2.5 cm}lllllP{4cm}p{4cm}}
\toprule
\textbf{Short name}&\textbf{Domain}&\textbf{Users}&\textbf{Items}&\textbf{Interactions}&\textbf{Sessions}&\textbf{Source}&\textbf{Used in}\\
\midrule
Amazon&E-commerce&20M&6M&143M&N/A&\citep{macauley15image}&\citep{he16fusing}\\
Epinions&E-commerce&40k&110k&181k&N/A&\citep{zhao14leveraging}&\citep{he16fusing}\\
Recsys Chall. 2015&E-commerce&N/A&38k&34M&9.5M&\citep{ben-shimon15recsys}&\citep{hidasi16session}\\
Ta-feng&E-commerce&32k&24k&829k&N/A&\url{recsyswiki.com/wiki/Grocery_shopping_datasets}&\citep{wang15basket,yu16dynamic}\\
T-Mall&E-commerce&1k&10k&5k&N/A&\url{ijcai-15.org/index.php/repeat-buyers-prediction-competition}&\citep{wang15basket,yu16dynamic}\\
AVITO&E-commerce&N/A&4k&767k&32k&\citep{twardowski16contextual}&\citep{twardowski16contextual}\\
\midrule
Microsoft&Web browsing&27k/13k&8k&13k/55k&32k/5k&\citep{breese98empirical}&\citep{zidmars01temporal,zhou04intelligent}\\
MSNBC&Web browsing&1.3M/87k&1k&476k/180k&N/A&\citep{cadez00visualization}&\citep{zidmars01temporal,yap12sequential}\\
Delicious&Web browsing&8.8k&3.3k&60k&45k&\citep{xiang10temporal}&\citep{xiang10temporal}\\
CiteULike&Web browsing&53k&1.8k&2.1M&40k&\citep{xiang10temporal}&\citep{xiang10temporal}\\
\midrule
AOL&Query&650k&N/A&17M&2.5M&\citep{sordoni15hierarchical}&\citep{sordoni15hierarchical}\\
\midrule
Foursquare 1&POI&31k&N/A&N/A&N/A&\citep{bao12location}&\citep{he16inferring}\\
Foursquare 2&POI&225k&N/A&22.5M&N/A&\citep{cheng11exploring}&\citep{cheng13where,he16fusing}\\
Gowalla 1&POI&54k&367k&4M&N/A&\citep{cheng12fused}&\citep{cheng13where,he16fusing}\\
Gowalla 2&POI&196k&N/A&6.4M&N/A&\citep{cho11friendship}&\citep{liu16next,liu16unified}\\
NYC Taxi Dataset&POI&N/A&299&N/A&670k&\citep{du16recurrent}&\citep{du16recurrent}\\
Global Terrorism Database&POI&N/A&N/A&N/A&N/A&\citep{liu16next}&\citep{liu16next}\\
\midrule
Art Of the Mix&Music&N/A&218k&N/A&29k&\citep{berenzweig04large}&\citep{hariri12context,mcfee11nlp,jannach15playlist}\\
30Music&Music&40k&5.6M&31M&2.7M&\citep{turrin1530music}&\citep{turrin15large,vasile16meta}\\
\bottomrule
\end{tabular}
\end{sidewaystable}
\end{comment}

\begin{sidewaystable}
\caption{Publicly available datasets for sequential recommendation. An updated version of this table with URLs is available at this link [ TODO: ADD LINK].}
\label{tab:datasets}
\footnotesize
\begin{tabular}{llllllP{6cm}}
\toprule
\textbf{Short name}&\textbf{Domain}&\textbf{Users}&\textbf{Items}&\textbf{Interactions}&\textbf{Sessions}&\textbf{Reference}\\
\midrule
Amazon&E-commerce&20M&6M&143M&N/A&\citep{he16fusing}\\
Epinions&E-commerce&40k&110k&181k&N/A&\citep{he16fusing}\\
Recsys Chall. 2015&E-commerce&N/A&38k&34M&9.5M&\citep{hidasi16session}\\
Ta-feng&E-commerce&32k&24k&829k&N/A&\citep{wang15basket,yu16dynamic}\\
T-Mall&E-commerce&1k&10k&5k&N/A&\citep{wang15basket,yu16dynamic}\\
AVITO&E-commerce&N/A&4k&767k&32k&\citep{twardowski16contextual}\\
\midrule
Microsoft&Web browsing&27k/13k&8k&13k/55k&32k/5k&\citep{zidmars01temporal,zhou04intelligent}\\
MSNBC&Web browsing&1.3M/87k&1k&476k/180k&N/A&\citep{zidmars01temporal,yap12sequential}\\
Delicious&Web browsing&8.8k&3.3k&60k&45k&\citep{xiang10temporal}\\
CiteULike&Web browsing&53k&1.8k&2.1M&40k&\citep{xiang10temporal}\\
\midrule
AOL&Query&650k&N/A&17M&2.5M&\citep{sordoni15hierarchical}\\
\midrule
Foursquare 1&POI&31k&N/A&N/A&N/A&\citep{he16inferring}\\
Foursquare 2&POI&225k&N/A&22.5M&N/A&\citep{cheng13where,he16fusing}\\
Gowalla 1&POI&54k&367k&4M&N/A&\citep{cheng13where,he16fusing}\\
Gowalla 2&POI&196k&N/A&6.4M&N/A&\citep{liu16next,liu16unified}\\
NYC Taxi Dataset&POI&N/A&299&N/A&670k&\citep{du16recurrent}\\
Global Terrorism Database&POI&N/A&N/A&N/A&N/A&\citep{liu16next}\\
\midrule
Art Of the Mix&Music&N/A&218k&N/A&29k&\citep{hariri12context,mcfee11nlp,jannach15playlist}\\
30Music&Music&40k&5.6M&31M&2.7M&\citep{turrin15large,vasile16meta}\\\bottomrule
\end{tabular}
\end{sidewaystable}
